Safety Synthesis Sans Specification

We define the problem of learning a transducer ${S}$ from a target language $U$ containing possibly conflicting transducers, using membership queries and conjecture queries. The requirement is that the language of ${S}$ be a subset of $U$. We argue that this is a natural question in many situations in hardware and software verification. We devise a learning algorithm for this problem and show that its time and query complexity is polynomial with respect to the rank of the target language, its incompatibility measure, and the maximal length of a given counterexample. We report on experiments conducted with a prototype implementation.

==> examples/example1/CSVs.tex <==















==> examples/example1/hyp0.tex <==
\begin{tikzpicture}[automaton]
  \small
  \node[state] (1) at(0,0) {};
  \node[state, right= of 1] (3) {};
  \node[initial, draw, circle, yshift=1cm] (0) at ($(1)!0.5!(3)$) {};
  \node at (0) {$\star$};
  \node at (1) {$g,\overline{g}$};
  \node at (3) {$g$};
  \path
    (0) edge node [above left] {$r,\overline{r}$} (1)
    (0) edge [above right] node [auto] {$\overline{r}$} (3)
    (1) edge [bend left=10] node [auto] {$r,\overline{r}$} (3)
    (3) edge [bend left=10] node [auto] {$r,\overline{r}$} (1);
\end{tikzpicture} 

==> examples/example1/table0.tex <==
\csvreader
[
    head to column names,
    tabular=l|l|ccc,
    separator=semicolon,
    table head={\toprule 
            \multicolumn{1}{c}{$\nabla$} &
            \multicolumn{1}{c}{\ttitle} &
            $\epsilon$ & 
            $r$ &
            $\overline{r}$
    },
    late after head=\\\midrule,
    before line={\ifnum\isbase<1\rowcolor{gray!30}\fi},
    table foot=\bottomrule
]
{\csvfile}{}{
    \bases &
    \prefix & 
    \eps &
    \pr & 
    \nr 
}

==> examples/example2/CSVs.tex <==

































==> examples/example2/hyp0.tex <==
\begin{tikzpicture}[automaton]
  \small
  \node[state] (1) at(0,0) {};
  \node[state, right= of 1] (3) {};
  \node[initial, draw, circle, yshift=1cm] (0) at ($(1)!0.5!(3)$) {};
  \node at (0) {$\specialsymbol$};
  \node at (1) {$\overline{g}$};
  \node at (3) {$g$};
  \path
    (0) edge node [above left] {$r$} (1)
    (0) edge node [above right] {$\overline{r}$} (3)
    (1) edge [bend left=10] node [auto] {$1$} (3)
    (3) edge [bend left=10] node [auto] {$1$} (1);
\end{tikzpicture} 

==> examples/example2/hyp1.tex <==
\begin{tikzpicture}[automaton]
  \small
  \node[state] (1) at(0,0) {};
  \node[state, right= of 1] (3) {};
  \node[initial, draw, circle, yshift=1cm] (0) at ($(1)!0.5!(3)$) {};
  \node at (0) {$\specialsymbol$};
  \node at (1) {$g$};
  \node at (3) {$\overline{g}$};
  \path
    (0) edge node [above left] {$1$} (1)
    (1) edge [bend left=10] node [auto] {$1$} (3)
    (3) edge [bend left=10] node [auto] {$1$} (1);
\end{tikzpicture} 

==> examples/example2/table0.tex <==
\csvreader
[
    head to column names,
    tabular=l|l|ccc,
    separator=semicolon,
    table head={\toprule 
            \multicolumn{1}{c}{$\nabla$} &
            \multicolumn{1}{c}{\ttitle} &
            $\epsilon$ & 
            $r$ &
            $\overline{r}$
    },
    late after head=\\\midrule,
    before line={\ifnum\isbase<1\rowcolor{gray!30}\fi},
    table foot=\bottomrule
]
{\csvfile}{}{
    \bases &
    \prefix & 
    \eps &
    \pr & 
    \nr 
}

==> examples/example3/CSVs.tex <==


















==> examples/example3/hyp0.tex <==
\begin{tikzpicture}[automaton]
  \small
  \node[initial, draw, circle] (0) at (0,0) {};
  \node[state, right=1.25cm of 0] (3) {};
  \node at (0) {$\star$};
  \node at (3) {$\{2\}$};
  \path
    (0) edge node [auto] {$a,b$} (3)
    (3) edge [loop right] node [auto] {$a,b$} (3);
\end{tikzpicture} 

==> examples/example3/table0.tex <==
\csvreader
[
    head to column names,
    tabular=l|l|c,
    separator=semicolon,
    table head={\toprule 
            \multicolumn{1}{c}{$\nabla$} &
            \multicolumn{1}{c}{\ttitle} &
            $\epsilon$
    },
    late after head=\\\midrule,
    before line={\ifnum\isbase<1\rowcolor{gray!30}\fi},
    table foot=\bottomrule
]
{\csvfile}{}{
    \bases &
    \prefix & 
    \eps
}

==> preamble/CSVs.tex <==





































































































































































==> preamble/authors.tex <==
%
\author{
    Roderick Bloem\inst{1} \and
    Hana Chockler\inst{2} \and\\
    Masoud Ebrahimi\inst{1} \and
    Dana Fisman\inst{3} \and
    Heinz Riener\inst{4}
    %Third Author\inst{3}\orcidID{2222--3333-4444-5555}
}
%
\authorrunning{R. Bloem et al.}
% First names are abbreviated in the running head.
% If there are more than two authors, 'et al.' is used.
%
\institute{
    ~\inst{1}~TU Graz \hspace{2mm}
    \inst{2}~King's College London \hspace{2mm}
    \inst{3}~Ben-Gurion University \hspace{2mm}
    \inst{4}~EPFL
}
%

==> sections/abstract.tex <==
\commentout{
\begin{abstract}
We examine the problem of synthesis of reactive systems, when the specification is unknown. 
We propose to replace synthesis by learning a system from a set of example traces.
The existing body of results regarding learning regular $\omega$-languages, essentially provides a way to learn a specification of a reactive system, rather than
a system itself. It thus does not provide an alternative for synthesis. The challenge in learning a system compared to learning a specification is that 
good examples can conform to different implementations. A learning algorithm should be able to cope with examples coming from possibly conflicting implementations and
still synthesize a system that meets the unknown specification.
We present a theoretical framework for synthesizing safety specifications in such a setting and its implementation in ***tool***. We discuss possible applications of our approach.
\keywords{First keyword  \and Second keyword \and Another keyword.}
\end{abstract}}


\begin{abstract}
We define the problem of learning a transducer $\aut{S}$ from a target language $U$ containing possibly conflicting transducers, using membership queries and conjecture queries.
The requirement is that the language of $\aut{S}$ be contained in $U$.
We argue that this is a natural question in many situations in hardware and software verification.
We devise a learning algorithm for this problem and show that its time and query complexity is polynomial with respect to the rank of the target language, its incompatibility measure, and
the maximal length of a given counterexample. We report on experiments conducted with a prototype implementation. 
\keywords{First keyword  \and Second keyword \and Another keyword.}
\end{abstract}

==> sections/algorithms/close.tex <==
\begin{algorithmic}[1]
\Require{Symbolic Table $\tab{T}=(R,C,M,B,\nabla)$}
\Ensure{Symbolic Table $\tab{T'}=(R',C,M,B',\nabla)$}
\Statex
\Function{\rm close}{\tab{T}}
    \Let{$R'$}{$R$}
    \Let{$B'$}{$B$}
    \ForAll {$r \in B\ialphit \setminus R$}
        \If{$\nexists b \in B: \text{covers}(M(b), M(r))$}
            \Push{$R'$}{$\{ r\sigma:\forall \sigma \in \Sigma\}$}
            \Push{$B'$}{$\{r\}$}
        \EndIf
    \EndFor
    \State \Return $(R',C,M,B',\nabla)$
\EndFunction
\end{algorithmic}

==> sections/algorithms/closed.tex <==
\begin{algorithm}
  \caption{Check if a symbolic table is closed.}
  \begin{algorithmic}[1]
    \Require{Symbolic Table $\tab{T}=(R,C,M,B,\nabla)$}
    \Ensure{$\ttt$ iff \tab{T} is closed.}
    \Statex
    \Function{\rm closed}{\tab{T}}
        \ForAll {$r \in B\ialphit \setminus R$}
            \If {$\nexists b \in B : \text{covers}(M(b), M(r))$}
                \State\Return \fff
            \EndIf
        \EndFor
        \State \Return \ttt
    \EndFunction
\end{algorithmic}
\end{algorithm}

==> sections/algorithms/cover.tex <==
\begin{algorithm}
  \caption{Compute the cover for a row \wrt a base.}
  \begin{algorithmic}[1]
    \Function{\rm cover}{$b, r$}
        \State \Return $b \to r$
    \EndFunction
\end{algorithmic}
\end{algorithm}

==> sections/algorithms/covers.tex <==
\begin{algorithm}
  \caption{Check if a base covers a row.}
  \begin{algorithmic}[1]
    \Function{\rm covers}{$b, r$}
        \If{all entries in $\text{cover}(b, r)$ are \ttt}
            \State \Return \ttt
        \EndIf
        \State \Return \fff
    \EndFunction
\end{algorithmic}
\end{algorithm}

==> sections/algorithms/deterministic.tex <==
% \documentclass[a4paper]{article}
% \input{premeable/packages.tex}
% \input{premeable/definitions.tex}
% \input{premeable/acronyms.tex}

% \begin{document}

\begin{algorithm}
  \caption{Check if a symbolic table induces a deterministic transducer.}
  \begin{algorithmic}[1]
    \Require{Symbolic Table $\tab{T}=(R,C,M,B,\nabla)$}
    \Ensure{$\ttt$ iff \tab{T} is deterministic.}
    \Statex
    \Function{\rm deterministic}{\tab{T}}
        \ForAll {$r \in B\ialphit \setminus R$}
            \If{$\nexists b \in B: \base{b} = \base{r}$}
                \State \Return \fff
            \EndIf
        \EndFor
        \State \Return minimal(\tab{T})
    \EndFunction
  \end{algorithmic}
\end{algorithm}

% \end{document}

==> sections/algorithms/determinize.tex <==
% \documentclass[a4paper]{article}
% \input{premeable/packages.tex}
% \input{premeable/definitions.tex}
% \input{premeable/acronyms.tex}

% \begin{document}

\begin{algorithm}
  \caption{Determinize a symbolic table.}
  \begin{algorithmic}[1]
    \Require{Symbolic Table $\tab{T}=(R, C, M, B, \nabla)$}
    \Ensure{Symbolic Table $\tab{T}=(R'\supseteq R, C'\supseteq C, M'\supseteq M, B' \supseteq B, \nabla')$}
    \Statex
    \Function{\rm determinize}{\tab{T}} 
        \Let{\tab{T'}}{\tab{T}} \Comment{$\tab{T'}$: a fresh copy of table \tab{T}.}
        \ForAll {$r \in B\ialphit \setminus R$}
            \If{$\exists b \in B: \base{b} = \base{r}$}
                \State \Continue
            \EndIf
            \Let{consistent}{\fff}
            \ForAll {$b_1,b_2 \in \base{r}$}
                \Let{$S$}{differentiate($b_1,b_2,\tab{T}$)}
                \If{$S \subset C$} \Continue\EndIf
                \ForAll{$c \in S \setminus C$}
                    %\Let{\tab{T''}}{$(R',C'\cup\{c\}, M', B', \nabla')$}
                    \Let{\tab{T''}}{fill($R',C'\cup\{c\}, M', B', \nabla'$)}
                    \Let{\tab{T''}}{rebase(\tab{T''})}
                    \If{$\exists b \in B : \nabla''(b) = \nabla''(r)$}
                        \Let{consistent}{\ttt}
                        \Let{\tab{T'}}{\tab{T''}}
                        \State \Break
                    \EndIf
                \EndFor
                \If{consistent} \Break \EndIf
            \EndFor
            \If{\textbf{not} consistent}
                \Push{$R'$}{$\{ r\sigma:\forall \sigma \in \Sigma\}$}
                \Push{$B'$}{$\{r\}$}
            \EndIf
        \EndFor
    \State \Return \tab{T'}
    \EndFunction

    % \Statex
    % \Function{\rm determinize}{$R, C, M, B, \nabla$}
    %     \ForAll {$r \in R \setminus B$}
    %         \If{$\exists b \in B: \base{b} = \base{r}$}
    %             \Continue
    %         \EndIf
    %         \If{$\exists b_1, b_2 \in \base{r}$ \st \textbf{not} satisfiable($M(b_1) \land M(b_2)$)}
    %             \Push{$R$}{$\{ r\sigma:\forall \sigma \in \Sigma\}$}
    %             \Push{$B$}{$\{r\}$}
    %             \State \Continue
    %         \EndIf
    %         \Let{consistent}{\fff}
    %         \ForAll {$b_1,b_2 \in \base{r}$}
    %             \Let{$S$}{differentiate($b_1,b_2,\tab{T}$)}
    %             \If{$S \subset C$} \Continue\EndIf
    %             \ForAll{$c \in S \setminus C$}
    %                 \Let{$(R,C',M',B,\nabla')$}
    %                     {rebase(fill($R,C\cup\{c\},M,B,\nabla$))}
    %                 \If{$\exists b \in B : \newbase{b} = \newbase{r}$}
    %                     \Let{$(C,M,\nabla,\text{consistent})$}
    %                         {$(C',M',\nabla',\ttt)$}
    %                     \State \Break
    %                 \EndIf
    %             \EndFor
    %             \If{consistent} \Break \EndIf
    %         \EndFor
    %         \If{\textbf{not} consistent}
    %             \Push{$R$}{$\{ r\sigma:\forall \sigma \in \Sigma\}$}
    %             \Push{$B$}{$\{r\}$}
    %         \EndIf
    %     \EndFor
    % \State \Return {$(R, C, M, B, \nabla)$}
    % \EndFunction
    
    % \Statex
    % \Function{\rm determinize}{\tab{T}} \Comment{\textcolor{red}{this is a more readable version of above.}}
    %     \Let{\tab{T'}}{\tab{T}} \Comment{$\tab{T'}$: a fresh copy of table \tab{T}.}
    %     \ForAll {$r \in R \setminus B$}
    %         \If{$\exists b \in B: \base{b} = \base{r}$}
    %             \Continue
    %         \EndIf
    %         \If{$\exists b_1, b_2 \in \base{r}$ \st \textbf{not} satisfiable($M(b_1) \land M(b_2)$)}
    %             \Push{$R'$}{$\{ r\sigma:\forall \sigma \in \Sigma\}$}
    %             \Push{$B'$}{$\{r\}$}
    %             \State \Continue
    %         \EndIf
    %         \Let{consistent}{\fff}
    %         \ForAll {$b_1,b_2 \in \base{r}$}
    %             \Let{$S$}{differentiate($b_1,b_2,\tab{T}$)}
    %             \If{$S \subset C$} \Continue\EndIf
    %             \ForAll{$c \in S \setminus C$}
    %                 %\Let{\tab{T''}}{$(R',C'\cup\{c\}, M', B', \nabla')$}
    %                 \Let{\tab{T''}}{fill($R',C'\cup\{c\}, M', B', \nabla'$)}
    %                 \Let{\tab{T''}}{rebase(\tab{T''})}
    %                 \If{$\exists b \in B : \nabla''(b) = \nabla''(r)$}
    %                     \Let{consistent}{\ttt}
    %                     \Let{\tab{T'}}{\tab{T''}}
    %                     \State \Break
    %                 \EndIf
    %             \EndFor
    %             \If{consistent} \Break \EndIf
    %         \EndFor
    %         \If{\textbf{not} consistent}
    %             \Push{$R'$}{$\{ r\sigma:\forall \sigma \in \Sigma\}$}
    %             \Push{$B'$}{$\{r\}$}
    %         \EndIf
    %     \EndFor
    % \State \Return \tab{T'}
    % \EndFunction
  \end{algorithmic}
\end{algorithm}

\begin{algorithm}
  \caption{Alternative determinization method for a symbolic table.}
  \begin{algorithmic}[1]
    \Require{Nondeterministic Symbolic Table $(R, C, M, B, \nabla)$}
    \Ensure{Deterministic Symbolic Table $(R', C', M', B', \nabla')$}
    \Statex
    \Function{\rm determinize}{$R, C, M, B, \nabla$}    
        \ForAll {$r \in R \setminus B$}
            \If{$\exists b \in B: \base{b} = \base{r}$}
                \State\Continue
            \EndIf
            \Let{$S$}{$\{\}$}
            \ForAll {$b_1,b_2 \in \base{r}$}
                \Push{$S$}{differentiate($b_1,b_2, \tab{T}$)}
            \EndFor
            \If{$S \subset C$}
                \Push{$R$}{$\{ r\cdot\sigma: \forall \sigma \in \Sigma\}$}
                \Push{$B$}{$\{ r \}$}
                \State\Continue
            \EndIf
            \Let{consistent}{\fff}
            \ForAll{$c \in S \setminus C$}
                \Let{$(R,C',M',B,\nabla')$}
                    {rebase(fill($R,C\cup\{c\},M,B,\nabla$))}
                \If{$\exists b \in B : \newbase{b} = \newbase{r}$}
                    \Let{$(C,M,\nabla,\text{consistent})$}
                        {$(C',M',\nabla',\ttt)$}
                    \State \Break
                \EndIf
            \EndFor
            \If{\textbf{not} consistent}
                \Push{$R$}{$\{ r\sigma: \forall \sigma \in \Sigma\}$}
                \Push{$B$}{$\{ r \}$}
            \EndIf
        \EndFor
    \State \Return {rebase($R, C, M, B, \nabla$)}
    \EndFunction
  \end{algorithmic}
\end{algorithm}

% \end{document}

==> sections/algorithms/differentiate.tex <==
\begin{algorithm}
  \caption{Find distinguishing suffixes for two bases in a symbolic table.}
  \begin{algorithmic}[1]
    \Require{Symbolic Table $\tab{T}=(R, C, M, B, \nabla)$, and $u, v \in B$}
    \Ensure{$S \subset \Sigma^*$}
    \Statex
    \Function{\rm differentiate}{$u, v, T$}
        \Let{$S$}{$\{ \}$} \Comment{$S:$ set of distinguishing suffixes.}
        \ForAll{$\sigma \in \Sigma$}
            % \Let{$u'$}{$u\sigma$}
            % \Let{$v'$}{$v\sigma$}
            \Let{$\mathcal{U}$}{$\{ M(u\sigma) \}$}
            \Let{$\mathcal{V}$}{$\{ M(v\sigma) \}$} 
            \If{$u\sigma \notin B$}
                \Let{$\mathcal{U}$}
                {$\{\text{cover}(M(b), M(u\sigma)) : \forall b \in \nabla(u\sigma) \}$}
            \EndIf
            \If{$v\sigma \notin B$}
                \Let{$\mathcal{V}$}
                {$\{ \text{cover}(M(b), M(v\sigma)) : \forall b \in \nabla(v\sigma) \}$}
            \EndIf
            \ForAll{$row \in \mathcal{U}$}
                \ForAll{$row' \in \mathcal{V}$}
                    \Push{$S$}{$\{ \sigma c : \forall c \in C \text{ \st } row\langle c \rangle \neq row' \langle c \rangle \}$}
                \EndFor
            \EndFor
        \EndFor
        \State \Return{$S$}
    \EndFunction
  \end{algorithmic}
\end{algorithm}

==> sections/algorithms/processCE.tex <==
\begin{algorithmic}[1]
    %\Require{$\smq_U$,$\ssq_U$,$\scq_U$,$\mq_U$ for an exhaustive bi-language $U$}
    %\Ensure{Automaton $\aut{A}$ implementing $U$}
    \Statex
    \Procedure{$\processCE}{$\set{H},\sytb{H}},\biword{\isym_1}{\osym_1}\biword{\isym_2}{\osym_2}\ldots \biword{\isym_\ell}{\osym_\ell}$}   
   
    \EndProcedure
 \end{algorithmic}




==> sections/algorithms/refine.tex <==
\begin{algorithm}
  \caption{Prefix based processing of a counterexample.}
  \begin{algorithmic}[1]
    \Require{A closed and deterministic $\tab{T}$, $\pi \in \{\ialph \times \bools(\oalph)\}^\omega$.}
    \Ensure{A list of symbolic tables.}
    \Statex
    \Function{\rm refine}{$\mathrm{T}, \pi$} 
        \Let{$\tab{T}'$}{$\tab{T}$}
            \Comment{$\tab{T}'$: a fresh copy of table \tab{T}.}
        \Let{$\langle \mu,\nu \rangle$}{$\pi$}
            \Comment{$\mu$: prefix, $\nu$: cycle.}
        \For{$n \leq |\mu| + |\nu|$}
            \Let{$\varrho$}{$\pi[..n]$}
                \Comment{$\varrho$: $\pi$'s prefix of length $n$.}%
            \ForAll{$r \vdash \project{\varrho}{\ialph}$}
                \Comment{$r$: input trace modeling $\project{\varrho}{\ialph}$.}
                \Push{$R'$}{$\{ r \}$}
            \EndFor
        \EndFor
        \Let{\tab{T'}}{fill(\tab{T'})}
        \Statex
        \Let{\set{T}}{$\{\}$}
        \ForAll{$r \in R'$}
            \ForAll{$c \in C'$}
                \Let{$\varrho$}{$\pi[..|rc|]$}
                    \Comment{$\varrho$: $\pi$'s prefix of length $|rc|$.}%
                \If{$rc \vdash \project{\varrho}{\ialph}$}
                    \Comment{if input trace $rc$ models $\project{\varrho}{\ialph}$.}
                    \Let{$\vartheta$}{$\project{\pi}{\oalph}[|rc|]$}
                        \Comment{$\vartheta$: output at position $|rc|$ of $\pi$.}
                    \Let{$\tab{T}''$}{$\tab{T}'$}
                        \Comment{$\tab{T}''$: a fresh copy of table \tab{T'}.}
                    \Let{$M''(r,c)$}{$M'(r,c) \land \neg \vartheta$}
                    \Comment{eliminate $\vartheta$ from $r\xrightarrow{c}$.}%
                \EndIf
            \EndFor
            \Push{\set{T}}{$\{\tab{T}''\}$}
        \EndFor
        \State\Return $\set{T}$
    \EndFunction
\end{algorithmic}
\end{algorithm}

% \begin{algorithm}
%   \caption{Prefix based processing of a counterexample.}
%   \begin{algorithmic}[1]
%     \Require{A closed and deterministic $\tab{T}$, $\pi \in \{\ialph \times \bools(\oalph)\}^\omega$.}
%     \Ensure{A list of symbolic tables.}
%     \Statex
%     \Function{\rm refine}{$\set{T}, \set{X}, \mathrm{T}, \pi$} \Comment{\textcolor{red}{This is incorrect, look below.}}
%         \Let{$(\mu,\nu)$}{$\pi$}
%             \Comment{$\pi=\mu(\nu)^\omega \text{ where } \mu, \nu \in \{\ialph\times\bools(\oalph)\}^*$.}
%         \Let{$\mathrm{\Theta}$}{$\{n : 1 \leq n \leq |\mu| + |\nu| \}$}
%         \Let{$\mathrm{\Xi}$}{$2^{\mathrm{\Theta}} \setminus \{\}$}
%         \Comment{$\mathrm{\Xi}$: set of all possible mutations.}
%         \Let{$(R,C,M,B,\nabla)$}{$\mathrm{T}$}
%         \ForAll{$\xi \in \mathrm{\Xi}$}
%             \Comment{$\xi$: current mutation}
%             \Let{$(R', M', B')$}{$(R, M, B)$}
%             \ForAll{$\langle r, c \rangle \in R \times C$}
%                 \If{$rc \notin \prefixes{\project{\pi}{\ialph}} \lor |rc| \notin \xi$}
%                     \State \Continue
%                 \EndIf
%                 \Let{$n$}{$|rc|$}
%                 \Let{$\vartheta$}{$(\project{\pi}{\oalph})[n]$}
%                 \Comment{$\vartheta$: symbolic output of $\pi[n]$}
%                 \Let{$\vartheta'$}{$M(r,c) \land \neg \vartheta$}
%                 \Comment{$\vartheta'$: new symbolic output}
%                 \Let{$M'(r,c)$}{$\vartheta'$}
%                 \If{$\vartheta' = \fff$}
%                     \Push{\set{X}}{$\{(R,C,M',B,\nabla)\}$} \Comment{forbid this mutation.}
%                     \Push{$R'$}{$\{ rc\sigma:\forall \sigma \in \Sigma\}$} 
%                     \Comment{explore new state.}
%                     \Push{$B'$}{$\{rc\}$} 
%                     \Let{$M'(r,c)$}{$\vartheta$}
%                     \Comment{revert output to $\vartheta$.}
%                 \EndIf
%             \EndFor
%             \Enqueue{\set{T}}{$\{(R',C,M',B',\nabla)\}$}
%         \EndFor
%         \State\Return $\set{T}, \set{X}$
%     \EndFunction
%     \Statex
%     \Function{\rm refine}{$\mathrm{T}, \pi$} \Comment{\textcolor{red}{This is also incorrect}}
%         \Let{\set{T}}{$\{\}$}
%         \ForAll{$r \in R$}
%             \ForAll{$c \in C$}
%                 \Let{$n$}{$|rc|$}
%                 \If{$rc \vdash \project{\pi}{\ialph}[..n]$}
%                     \State \Continue
%                 \EndIf
%                 \Let{$q$}{state$(r, \tab{T})$}
%                     \Comment{$q$: state from which $x$ emanates.}
%                 \Let{$\vartheta$}{$\project{\pi}{\oalph}[n]$}
%                     \Comment{$\vartheta$: output at position $n$ of $\pi$.}
%                 \Let{$\tab{T}'$}{$\tab{T}$}
%                     \Comment{$\tab{T}'$: a fresh copy of table \tab{T}.}
%                 \Let{$M'(q,c)$}{$M(q,c) \land \neg \vartheta$}
%                 \Comment{eliminate $\vartheta$ from $q\xrightarrow{c}$.}
%                 \If{$r \neq q \land M'(q,c) = \fff$}
%                     \Let{$M'(r,c)$}{$M'(q,c)$}                
%                         \Comment{eliminate $\vartheta$ from $r\xrightarrow{c}$.}
%                     \Let{$M'(q,c)$}{$M(q,c)$}                
%                         \Comment{previous output on $q\xrightarrow{c}$.}%
%                 \EndIf
%             \EndFor
%             \If{$\tab{T} \neq \tab{T'}$}
%                 \Push{\set{T}}{$\{\tab{T}'\}$}
%             \EndIf
%         \EndFor
%         \State\Return $\set{T}$
%     \EndFunction
% \end{algorithmic}
% \end{algorithm}

% % \begin{algorithm}
% %   \caption{Suffix based processing of a counterexample.}
% %   \begin{algorithmic}[1]
% %     \Require{Symbolic generator $(R,C,M,B,\nabla)$, $\pi \in \Sigma^\omega$, and $\varrho \in \bools(\Gamma)^\omega$.}
% %     \Ensure{A list of symbolic generators}
% %     \Statex
% %     \Function{$\alpha$}{$\pi, i$}
% %         \Let{$(\mu,\nu)$}{$\pi$}
% %             \Comment{$\pi=\mu(\nu)^\omega \text{ where } \mu, \nu \in \{\ialph\times\bools(\oalph)\}^*$.}
% %         \Let{$n$}{$|\mu|+|\nu|$}
% %         \Let{$\hat{\iota}$}{$i-1$}
% %         \If{$i \in \{0, n\}$}
% %             \State \Return $i = n$
% %         \EndIf
% %         \Let{$w$}{$\delta(\epsilon,(\project{\pi}{\ialph})[..\hat{\iota}])$}
% %         \If{$\smq(w\pi[i..n]) \leftrightarrow \smq(\pi[..n])$}
% %             \State \Return \ttt
% %         \EndIf
% %         \State \Return \fff
% %     \EndFunction
% %     \Statex
% %     \Function{\rm refine}{$\set{T}, \set{R}, \aut{A}, \mathrm{T}, \pi$}
% %         \Let{\set{T}}{$\{\}$} 
% %             \Comment{\set{T}: set of refined symbolic tables.}
% %         \Let{$\mathrm{\Theta}$}{$\{n : 0 < n \leq \lvert \pi \rvert \}$}
% %         \Let{$\mathrm{\Xi}$}{$2^{\mathrm{\Theta}} \setminus \{\}$}
% %         \Comment{$\mathrm{\Xi}$: set of all possible mutations.}
% %         \ForAll{$\xi \in \mathrm{\Xi}$}
% %             \Comment{$\xi$: a mutation set}
% %             \Let{$(R', M', B')$}{$(R, M, B)$}
% %             \ForAll{$r \in R$ \textbf{and} $c \in C$}
% %                 \If{$r\cdot c \in \prefixes{\pi}$}
% %                     \Let{$n$}{$\lvert r\cdot c \rvert$}
% %                     \If{$n \in \xi$} \Comment{if must mutate $M(r, c)$}
% %                         \If{$M(r,c) \land \neg \varrho^n \neq \fff$}
% %                             \Comment{if $\varrho^n$ is a wrong output}
% %                             \Let{$M'(r,c)$}{$M(r,c) \land \neg \varrho^n$}
% %                             \Comment{eliminate $\varrho^n$}
% %                         \Else \Comment{if $\varrho^n$ is the only output}
% %                             % \Let{$S$}{differentiate$(R,C',M',B,\nabla,\pi, r\cdot c)$}
% %                             % \Push{$C'$}{$S$}
% %                             \Push{$R'$}{$\{ (r\cdot c) \cdot \sigma:\forall \sigma \in \Sigma\}$}
% %                             \Push{$B'$}{$\{r\cdot c\}$}
% %                             \Comment{explore a potential state}
% %                             % \State \Break
% %                         \EndIf
% %                     \EndIf
% %                 \EndIf
% %             \EndFor
% %             \Push{\set{T}}{$(R',C,M',B',\nabla)$}
% %         \EndFor
% %         \State\Return $\mathbf{T}$
% %     \EndFunction
% % \end{algorithmic}
% \end{algorithm}

==> sections/algorithms/state.tex <==
\begin{algorithm}
  \caption{Find the access word to the state reached by an input word \label{alg:state}}
  \begin{algorithmic}[1]
    \Require{input word $\iw$, Symbolic Table \tab{T}}
    \Ensure{$b \in \ialph^*$}
    \Statex
    \Function{\rm state}{$\iw, \tab{T}$}
        \ForAll{$b \in B$}
            \If{$\base{b} = \base{\iw}$}
                \State \Return $b$
            \EndIf
        \EndFor
        \State \Return $\iw$
    \EndFunction
    \end{algorithmic}
\end{algorithm}

==> sections/algorithms/transducer.tex <==
\begin{algorithm}
  \caption{Extracting a transducer from a symbolic table.}
  \begin{algorithmic}[1]
    \Require{A closed and deterministic $\tab{T}=(R,C,M,B,\nabla)$.}
    \Ensure{A Symbolic Transducer $\aut{A}=(\ialph, \oalph, Q, \epsilon, \delta)$.}
    \Statex
    \Function{\rm transducer}{\tab{T}}
        \Let{$Q$}{$\{\epsilon\}$}
            \Comment{$Q$: transducer's state set}
        \Let{\set{X}}{$\{\}$}
            \Comment{\set{X}: processed states}
        \ForAll{$q \in Q \setminus \set{X}$}
            \Comment{for each unprocessed state $q$}
            \ForAll{$\isym \in \ialph$}
                \Let{$q'$}{state$(q\isym,\tab{T})$}
                \Let{$\vartheta$}{$M(q,\isym)$}
                \Let{$\delta(q, \isym)$}{$\langle q', \vartheta \rangle$}
                \Push{$Q$}{$\{q'\}$}
            \EndFor
            \Push{\set{X}}{$\{q\}$}
        \EndFor
        \State \Return ($\ialph, \oalph, Q, \epsilon, \delta$)
    \EndFunction
\end{algorithmic}
\end{algorithm}
